Less Is Harder Than More: Proving Unnecessary Complexity

When can a sensor, feature, or API field be removed without changing a fixed system's decisions? We require the remaining inputs to recover its complete optimal-action set, including ties, at every admitted state. Admitting every input combination guarantees one smallest preserving set. Yet checking one deletion is coNP-complete when circuits give utilities on Boolean products, even with two actions and at most two optimal-action sets. Missing combinations permit alternative preserving sets, so an auditor must choose inputs within budget and check the chosen set. Requiring every declared reading to have a positive-probability state adds a support check. We classify choosing and checking exactly for circuit-defined Boolean models, with and without the support requirement. A unique winner after averaging hidden states can still change the original decisions. Certifying such winners requires weighted score comparisons: finding inputs within budget is $\mathsf{NP}^{(\mathsf{NP}^{\mathsf{PP}})}$-complete even with two actions and independent uniform inputs. Explicit tables admit logarithmic approximation of the minimum preserving input count; succinct Boolean products admit no polynomial-time $o(\Lambda/\log\Lambda)$ approximation in total encoded length $\Lambda$, unless $\mathsf P=\mathsf{NP}$. Supplied decompositions and symmetry proofs can make audits polynomial-time; discovery and validation are additional work. For a frozen digit classifier, eleven blocks suffice on held-out rows but fifteen are needed on the full product; four conflicting pairs expose the gap. Building the required response from retained inputs establishes sufficiency, not minimality. Preserve the structure that makes the dependence checkable.

==> experiments/task_arrival/reproduced_gate1_20260915/generated/constrained_decoding_summary.tex <==
% Generated by constrained_decoding_audit.py; do not edit.
\newcommand{\decodingPromptCount}{12}
\newcommand{\decodingActionCount}{8}
\newcommand{\decodingTaskCount}{3}
\newcommand{\decodingOrderCount}{6}
\newcommand{\decodingTransitionCount}{12}
\newcommand{\decodingModelLockCount}{9}
\newcommand{\decodingUnavoidableLockCount}{9}
\newcommand{\decodingModelRecourseCount}{9}
\newcommand{\decodingUnavoidableRecourseCount}{9}
\newcommand{\decodingModelRecourseExcessCount}{4}
\newcommand{\decodingMaxModelPenalty}{0.333}
\newcommand{\decodingMaxUnavoidablePenalty}{0.333}
\newcommand{\decodingMaxModelRecourse}{0.667}
\newcommand{\decodingMaxModelRecourseExcess}{0.167}
\newcommand{\decodingMaxMipGap}{1.8e-16}
\newcommand{\decodingClassificationTolerance}{10^{-6}}
\newcommand{\decodingModelRevisionShort}{2290a626}


==> external_labels_ba09e5c155bb36b9.tex <==
% Generated from freshly compiled external-document labels. Do not edit.
% Numbers, pages and titles only: arXiv merges separately compiled PDFs.
\makeatletter
\newlabel{app:reproducibility-checklist}{{12}{57}{Reproducibility Checklist for JAIR}{}{}}
\newlabel{app:reproducibility-checklist@cref}{{[section][12][]12}{[1][57][]57}{}{}{}}
\newlabel{cor:free-top-unique-bottom}{{2.12}{7}{Full Interface and Smallest Sufficient Interface}{}{}}
\newlabel{cor:free-top-unique-bottom@cref}{{[theorem][12][2]2.12}{[1][7][]7}{}{}{}}
\newlabel{cor:joint-preservation-complexity}{{6.30}{35}{Complexity of Preserving Every Declared State}{}{}}
\newlabel{cor:joint-preservation-complexity@cref}{{[theorem][30][6]6.30}{[1][35][]35}{}{}{}}
\newlabel{cor:markov-blanket-support-boundary}{{6.16}{27}{When a Markov Blanket Matches Input Sufficiency}{}{}}
\newlabel{cor:markov-blanket-support-boundary@cref}{{[theorem][16][6]6.16}{[1][27][]27}{}{}{}}
\newlabel{cor:markov-blanket-uniqueness}{{6.17}{28}{Full-Support Blanket Uniqueness and Sparse-Support Failure}{}{}}
\newlabel{cor:markov-blanket-uniqueness@cref}{{[theorem][17][6]6.17}{[1][28][]28}{}{}{}}
\newlabel{cor:positive-gap-tolerance}{{2.15}{9}{Positive-Gap Tolerance Band}{}{}}
\newlabel{cor:positive-gap-tolerance@cref}{{[theorem][15][2]2.15}{[1][9][]9}{}{}{}}
\newlabel{cor:stochastic-preservation-relevance}{{6.27}{32}{Relevance and Positive Support}{}{}}
\newlabel{cor:stochastic-preservation-relevance@cref}{{[theorem][27][6]6.27}{[1][32][]32}{}{}{}}
\newlabel{cor:succinct-input-length-inapproximation}{{6.40}{41}{Input-Length Inapproximability}{}{}}
\newlabel{cor:succinct-input-length-inapproximation@cref}{{[theorem][40][6]6.40}{[1][41][]41}{}{}{}}
\newlabel{def:coordinate-presentation}{{2.2}{5}{Finite Coordinate Presentation}{}{}}
\newlabel{def:coordinate-presentation@cref}{{[theorem][2][2]2.2}{[1][5][]5}{}{}{}}
\newlabel{def:decision-equiv}{{2.5}{5}{Optimizer Quotient}{}{}}
\newlabel{def:decision-equiv@cref}{{[theorem][5][2]2.5}{[1][5][]5}{}{}{}}
\newlabel{def:decision-problem}{{2.1}{5}{Decision Problem}{}{}}
\newlabel{def:decision-problem@cref}{{[theorem][1][2]2.1}{[1][5][]5}{}{}{}}
\newlabel{def:decision-quotient}{{2.5}{5}{Optimizer Quotient}{}{}}
\newlabel{def:decision-quotient@cref}{{[theorem][5][2]2.5}{[1][5][]5}{}{}{}}
\newlabel{def:deployable-preservation}{{6.12}{25}{Input Sufficiency with Observation Coverage}{}{}}
\newlabel{def:deployable-preservation@cref}{{[theorem][12][6]6.12}{[1][25][]25}{}{}{}}
\newlabel{def:minimal-sufficient}{{2.8}{6}{Minimal Sufficient Set}{}{}}
\newlabel{def:minimal-sufficient@cref}{{[theorem][8][2]2.8}{[1][6][]6}{}{}{}}
\newlabel{def:optimizer}{{2.4}{5}{Optimizer Map}{}{}}
\newlabel{def:optimizer@cref}{{[theorem][4][2]2.4}{[1][5][]5}{}{}{}}
\newlabel{def:paired-tautology-family}{{6.37}{40}{Paired Tautology Family}{}{}}
\newlabel{def:paired-tautology-family@cref}{{[theorem][37][6]6.37}{[1][40][]40}{}{}{}}
\newlabel{def:pomdp-certification-contracts}{{7.4}{47}{Multistep Certification Contracts}{}{}}
\newlabel{def:pomdp-certification-contracts@cref}{{[theorem][4][7]7.4}{[1][47][]47}{}{}{}}
\newlabel{def:pomdp-history-semantics}{{7.3}{47}{Decision Histories and Optimizers}{}{}}
\newlabel{def:pomdp-history-semantics@cref}{{[theorem][3][7]7.3}{[1][47][]47}{}{}{}}
\newlabel{def:pomdp-succinct-interface}{{7.2}{46}{Succinct Unary-Horizon POMDP Encoding}{}{}}
\newlabel{def:pomdp-succinct-interface@cref}{{[theorem][2][7]7.2}{[1][46][]46}{}{}{}}
\newlabel{def:projection}{{2.3}{5}{Projection}{}{}}
\newlabel{def:projection@cref}{{[theorem][3][2]2.3}{[1][5][]5}{}{}{}}
\newlabel{def:relevant}{{2.10}{7}{Relevant Coordinate}{}{}}
\newlabel{def:relevant@cref}{{[theorem][10][2]2.10}{[1][7][]7}{}{}{}}
\newlabel{def:sequential-decision-problem}{{6.46}{44}{Sequential Decision Problem}{}{}}
\newlabel{def:sequential-decision-problem@cref}{{[theorem][46][6]6.46}{[1][44][]44}{}{}{}}
\newlabel{def:sequential-sufficient}{{6.47}{44}{Sequential Sufficiency}{}{}}
\newlabel{def:sequential-sufficient@cref}{{[theorem][47][6]6.47}{[1][44][]44}{}{}{}}
\newlabel{def:stochastic-anchor-sufficient}{{6.13}{25}{One Conditional Winner}{}{}}
\newlabel{def:stochastic-anchor-sufficient@cref}{{[theorem][13][6]6.13}{[1][25][]25}{}{}{}}
\newlabel{def:stochastic-decision-problem}{{6.10}{24}{Stochastic Decision Problem}{}{}}
\newlabel{def:stochastic-decision-problem@cref}{{[theorem][10][6]6.10}{[1][24][]24}{}{}{}}
\newlabel{def:stochastic-preservation}{{6.11}{24}{Preservation on Supported and Declared States}{}{}}
\newlabel{def:stochastic-preservation@cref}{{[theorem][11][6]6.11}{[1][24][]24}{}{}{}}
\newlabel{def:stochastic-singleton-sufficient}{{6.13}{25}{One Conditional Winner}{}{}}
\newlabel{def:stochastic-singleton-sufficient@cref}{{[theorem][13][6]6.13}{[1][25][]25}{}{}{}}
\newlabel{def:sufficient}{{2.7}{6}{Sufficient Coordinate Set}{}{}}
\newlabel{def:sufficient@cref}{{[theorem][7][2]2.7}{[1][6][]6}{}{}{}}
\newlabel{def:validity-promise-convention}{{3.1}{10}{Promise-Problem Convention}{}{}}
\newlabel{def:validity-promise-convention@cref}{{[theorem][1][3]3.1}{[1][10][]10}{}{}{}}
\newlabel{eq:gapp-signed-path-normal-form}{{5}{37}{Exact Two-Action Classification}{}{}}
\newlabel{eq:gapp-signed-path-normal-form@cref}{{[equation][5][]5}{[1][37][]37}{}{}{}}
\newlabel{eq:nested-fixed-block-source}{{4}{36}{One Threshold for Every Observation}{}{}}
\newlabel{eq:nested-fixed-block-source@cref}{{[equation][4][]4}{[1][36][]36}{}{}{}}
\newlabel{eq:preservation-minimum-collapse}{{2}{34}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{eq:preservation-minimum-collapse@cref}{{[equation][2][]2}{[1][34][]34}{}{}{}}
\newlabel{eq:stochastic-preservation-normal-form}{{1}{32}{Preservation Can Hold Without Observation Coverage}{}{}}
\newlabel{eq:stochastic-preservation-normal-form@cref}{{[equation][1][]1}{[1][31][]32}{}{}{}}
\newlabel{eq:weak-majority-convention}{{3}{35}{One Fiber: Equality Versus a Threshold}{}{}}
\newlabel{eq:weak-majority-convention@cref}{{[equation][3][]3}{[1][35][]35}{}{}{}}
\newlabel{ex:pomdp-two-step-noncomposition}{{7.1}{45}{One-step constancy does not compose through a belief update}{}{}}
\newlabel{ex:pomdp-two-step-noncomposition@cref}{{[theorem][1][7]7.1}{[1][45][]45}{}{}{}}
\newlabel{ex:sensor-support-contract}{{6.14}{25}{Supported and Declared-State Sensor Retention}{}{}}
\newlabel{ex:sensor-support-contract@cref}{{[theorem][14][6]6.14}{[1][25][]25}{}{}{}}
\newlabel{ex:treewidth-factorization}{{4.2}{13}{A tree-factored diagnostic decision}{}{}}
\newlabel{ex:treewidth-factorization@cref}{{[theorem][2][4]4.2}{[1][13][]13}{}{}{}}
\newlabel{ex:two-move-sequential-separation}{{6.44}{43}{A coordinate revealed after two moves}{}{}}
\newlabel{ex:two-move-sequential-separation@cref}{{[theorem][44][6]6.44}{[1][43][]43}{}{}{}}
\newlabel{fig:audit-procedure}{{5}{16}{A preservation audit has three outcomes: a certificate, a conflicting pair, or no verdict. Minimality, support coverage, and decisiveness require their own checks}{}{}}
\newlabel{fig:audit-procedure@cref}{{[figure][5][]5}{[1][15][]16}{}{}{}}
\newlabel{fig:diagnostic-summaries}{{4}{14}{More structure, cheaper audit. Each summary bit records whether all checks in its subtree pass. Two copies search for states with the same retained inputs but different actions. Finding a pair refutes deletion; exhausting this search without one certifies preservation. For the tree-factored utility in Example~\ref {ex:treewidth-factorization}, dynamic programming combines bounded-size bags in linear time at fixed branching, without enumerating all state pairs}{}{}}
\newlabel{fig:diagnostic-summaries@cref}{{[figure][4][]4}{[1][13][]14}{}{}{}}
\newlabel{fig:future-information}{{8}{46}{A sensor can matter later even when today's action is the same in both states. The bit $h$ is equally likely to be zero or one. Guessing it correctly pays one; a wrong guess pays zero. Keeping it makes continuation worth one. Hiding it at both decisions reduces that value to $1/2$, below the exit reward $3/4$. Thick green branches mark the best initial actions}{}{}}
\newlabel{fig:future-information@cref}{{[figure][8][]8}{[1][46][]46}{}{}{}}
\newlabel{fig:input-deletion}{{1}{2}{A definite choice can still lose a required answer. Deleting $x_2$ merges 00 (brake) with 01 (steer). No choice based on $x_1$ alone can recover both original decisions. Averaging selects brake for this group and continue for the other: decisiveness holds, but preservation fails}{}{}}
\newlabel{fig:input-deletion@cref}{{[figure][1][]1}{[1][2][]2}{}{}{}}
\newlabel{fig:learned-policy-scope-audit}{{2}{3}{Same classifier, different certificate scope. Eleven blocks suffice on the held-out inputs; fifteen are necessary on all admitted combinations. The two arrays disagree only in the top-left block, which the eleven-block interface omits, but receive different predictions. They refute that deletion on the product. Grid labels number blocks from one to sixteen; array entries are quantized input values}{}{}}
\newlabel{fig:learned-policy-scope-audit@cref}{{[figure][2][]2}{[1][3][]3}{}{}{}}
\newlabel{fig:missing-combinations}{{3}{8}{Missing combinations can hide a coordinate's relevance. On the left, either input distinguishes the two listed states. On the right, the newly admitted states have thick borders. Each outlined column groups states agreeing on $x_2$ but requiring different actions. The unique smallest sufficient set is now $\{1\}$}{}{}}
\newlabel{fig:missing-combinations@cref}{{[figure][3][]3}{[1][8][]8}{}{}{}}
\newlabel{fig:paired-selector-gadget}{{7}{39}{The two-action selector for Theorem~\ref {prop:two-action-exact-counting}, item~\ref {item:two-action-budget}. Left: each four-valued input carries a sign and an observation bit; omitting an entire pair leaves a cancelling hidden sign, so the budget chooses one input per pair. Middle: hidden assignments inconsistent with that choice cancel; the chosen assignment contributes its signed count. Right: the two action scores tie exactly when that count is zero. Testing every threshold index excludes every count below weak majority. All coordinates are independent and uniform}{}{}}
\newlabel{fig:paired-selector-gadget@cref}{{[figure][7][]7}{[1][38][]39}{}{}{}}
\newlabel{fig:support-contracts}{{6}{27}{The same interlock gives different preservation verdicts. Boxes group states that look the same through the retained inputs. Keeping one sensor recovers the actions on the support; keeping both recovers them at every declared state under the zero-score convention. Neither interface is both sufficient and observation-covering: the first mixes pointwise labels, and the second declares unsupported observations}{}{}}
\newlabel{fig:support-contracts@cref}{{[figure][6][]6}{[1][26][]27}{}{}{}}
\newlabel{item:two-action-budget}{{3}{38}{Exact Two-Action Decisiveness Classification}{}{}}
\newlabel{item:two-action-budget@cref}{{[enumi][3][]3}{[1][38][]38}{}{}{}}
\newlabel{item:two-action-check}{{1}{38}{Exact Two-Action Decisiveness Classification}{}{}}
\newlabel{item:two-action-check@cref}{{[enumi][1][]1}{[1][38][]38}{}{}{}}
\newlabel{item:two-action-some}{{2}{38}{Exact Two-Action Decisiveness Classification}{}{}}
\newlabel{item:two-action-some@cref}{{[enumi][2][]2}{[1][38][]38}{}{}{}}
\newlabel{lem:intersection-closure-collapse}{{2.9}{6}{Intersection Closure Gives a Least Member}{}{}}
\newlabel{lem:intersection-closure-collapse@cref}{{[theorem][9][2]2.9}{[1][6][]6}{}{}{}}
\newlabel{lem:majority-as-universal-nonzero}{{6.34}{37}{A Threshold Is a Family of Nonzero Tests}{}{}}
\newlabel{lem:majority-as-universal-nonzero@cref}{{[theorem][34][6]6.34}{[1][37][]37}{}{}{}}
\newlabel{lem:nested-pp-oracle-normal-form}{{6.33}{36}{One Threshold for Every Observation}{}{}}
\newlabel{lem:nested-pp-oracle-normal-form@cref}{{[theorem][33][6]6.33}{[1][36][]36}{}{}{}}
\newlabel{lem:pomdp-polynomial-space}{{7.5}{48}{Polynomial-Space Exact Continuation}{}{}}
\newlabel{lem:pomdp-polynomial-space@cref}{{[theorem][5][7]7.5}{[1][48][]48}{}{}{}}
\newlabel{lem:pomdp-sign-core}{{7.6}{48}{Sign-Separated QBF Planning Core}{}{}}
\newlabel{lem:pomdp-sign-core@cref}{{[theorem][6][7]7.6}{[1][48][]48}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:1}{{2.2}{5}{Recovering Responses from Retained Inputs}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:10}{{2.3}{7}{Sufficiency and Relevance}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:100}{{7}{49}{Why this holds}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:100@cref}{{[section][7][]7}{[1][49][]49}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:101}{{58}{49}{Unary-Horizon Interface Certification Is PSPACE-Complete}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:101@cref}{{[footnote][58][]58}{[1][49][]49}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:102}{{7}{49}{Why this holds}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:102@cref}{{[section][7][]7}{[1][49][]49}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:103}{{59}{49}{Horizon-Two Inheritance}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:103@cref}{{[footnote][59][]59}{[1][49][]49}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:104}{{60}{50}{Explicit-state baseline}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:104@cref}{{[footnote][60][]60}{[1][50][]50}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:105}{{61}{51}{Explicit-state baseline}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:105@cref}{{[footnote][61][]61}{[1][50][]51}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:10@cref}{{[subsection][3][2]2.3}{[1][7][]7}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:11}{{6}{7}{Listed States and Product Closure}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:11@cref}{{[footnote][6][]6}{[1][7][]7}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:12}{{7}{8}{Sufficiency and Relevance}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:12@cref}{{[footnote][7][]7}{[1][8][]8}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:13}{{8}{8}{Changing a setting is not removing a channel}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:13@cref}{{[footnote][8][]8}{[1][8][]8}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:14}{{2.4}{8}{Admissible Outputs}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:14@cref}{{[subsection][4][2]2.4}{[1][8][]8}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:15}{{9}{8}{Admissible Outputs as an Optimizer Quotient}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:15@cref}{{[footnote][9][]9}{[1][8][]8}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:16}{{2.4}{9}{Admissible Outputs}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:16@cref}{{[subsection][4][2]2.4}{[1][9][]9}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:17}{{10}{9}{Positive-Gap Tolerance Band}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:17@cref}{{[footnote][10][]10}{[1][9][]9}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:18}{{11}{11}{Algorithms and Structural Certificates}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:18@cref}{{[footnote][11][]11}{[1][11][]11}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:19}{{12}{12}{Two Direct Decomposition Checks}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:19@cref}{{[footnote][12][]12}{[1][11][]12}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:1@cref}{{[subsection][2][2]2.2}{[1][5][]5}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:2}{{1}{6}{Kernel Factorization for the Optimizer Map}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:20}{{4.2}{12}{Bounded Treewidth}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:20@cref}{{[subsection][2][4]4.2}{[1][12][]12}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:21}{{13}{12}{Bounded-Width CSP for Violating State Pairs}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:21@cref}{{[footnote][13][]13}{[1][12][]12}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:22}{{14}{14}{Coordinate Symmetry and Histogram Certificates}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:22@cref}{{[footnote][14][]14}{[1][14][]14}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:23}{{4.3}{15}{Coordinate Symmetry and Histogram Certificates}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:23@cref}{{[subsection][3][4]4.3}{[1][15][]15}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:24}{{15}{15}{Orbit Representatives and the Histogram Certificate}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:24@cref}{{[footnote][15][]15}{[1][15][]15}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:25}{{16}{15}{Coordinate Symmetry and Histogram Certificates}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:25@cref}{{[footnote][16][]16}{[1][15][]15}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:26}{{6.1.1}{20}{Product Closure Removes the Coordinate Choice}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:26@cref}{{[subsubsection][1][6,1]6.1.1}{[1][20][]20}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:27}{{17}{20}{One-Coordinate Deletion Is coNP-Complete}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:27@cref}{{[footnote][17][]17}{[1][20][]20}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:28}{{6.1.1}{21}{Quotient cardinality}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:28@cref}{{[subsubsection][1][6,1]6.1.1}{[1][21][]21}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:29}{{18}{21}{Finding a Sufficient Set Within Budget Is coNP-Complete}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:29@cref}{{[footnote][18][]18}{[1][21][]21}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:2@cref}{{[footnote][1][]1}{[1][5][]6}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:3}{{2}{6}{Sufficiency and Relevance}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:30}{{6.1.2}{21}{Missing Combinations Restore the Coordinate Choice}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:30@cref}{{[subsubsection][2][6,1]6.1.2}{[1][21][]21}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:31}{{19}{21}{Missing Combinations Keep the Choice Alive}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:31@cref}{{[footnote][19][]19}{[1][21][]21}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:32}{{6.1.3}{23}{One Observation and an Existential--Universal Check}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:32@cref}{{[subsubsection][3][6,1]6.1.3}{[1][23][]23}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:33}{{20}{23}{Finding One Observation That Preserves the Answer}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:33@cref}{{[footnote][20][]20}{[1][23][]23}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:34}{{6.3}{27}{Markov Blankets and Preservation on Supported States}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:34@cref}{{[subsection][3][6]6.3}{[1][27][]27}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:35}{{21}{27}{Optimizer Markov-Blanket Equivalence}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:35@cref}{{[footnote][21][]21}{[1][27][]27}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:36}{{6.3}{27}{Markov Blankets and Preservation on Supported States}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:36@cref}{{[subsection][3][6]6.3}{[1][27][]27}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:37}{{22}{27}{When a Markov Blanket Matches Input Sufficiency}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:37@cref}{{[footnote][22][]22}{[1][27][]27}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:38}{{6.3}{28}{Markov Blankets and Preservation on Supported States}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:38@cref}{{[subsection][3][6]6.3}{[1][28][]28}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:39}{{23}{28}{Full-Support Blanket Uniqueness and Sparse-Support Failure}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:39@cref}{{[footnote][23][]23}{[1][28][]28}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:3@cref}{{[footnote][2][]2}{[1][6][]6}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:4}{{2.3}{6}{Sufficiency and Relevance}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:40}{{6.4}{28}{Intersection Closure Governs Within-Budget Certification}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:40@cref}{{[subsection][4][6]6.4}{[1][28][]28}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:41}{{24}{28}{Intersection Closure Separates Preservation from Decisiveness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:41@cref}{{[footnote][24][]24}{[1][28][]28}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:42}{{25}{29}{Preservation without Decisiveness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:42@cref}{{[footnote][25][]25}{[1][29][]29}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:43}{{26}{29}{Decisiveness without Preservation}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:43@cref}{{[footnote][26][]26}{[1][29][]29}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:44}{{6.5.3}{30}{Sparse Support Keeps the Blanket Choice Alive}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:44@cref}{{[subsubsection][3][6,5]6.5.3}{[1][30][]30}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:45}{{27}{30}{Sparse Support Keeps the Blanket Choice Alive}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:45@cref}{{[footnote][27][]27}{[1][30][]30}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:46}{{28}{31}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:46@cref}{{[footnote][28][]28}{[1][31][]31}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:47}{{29}{31}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:47@cref}{{[footnote][29][]29}{[1][31][]31}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:48}{{6.5.4}{31}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:48@cref}{{[subsubsection][4][6,5]6.5.4}{[1][31][]31}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:49}{{30}{31}{Full Support Reduces Preservation to Input Sufficiency}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:49@cref}{{[footnote][30][]30}{[1][31][]31}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:4@cref}{{[subsection][3][2]2.3}{[1][6][]6}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:5}{{3}{6}{Intersection Closure Gives a Least Member}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:50}{{31}{31}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:50@cref}{{[footnote][31][]31}{[1][31][]31}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:51}{{6.5.4}{31}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:51@cref}{{[subsubsection][4][6,5]6.5.4}{[1][31][]31}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:52}{{32}{32}{Preservation Can Hold Without Observation Coverage}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:52@cref}{{[footnote][32][]32}{[1][31][]32}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:53}{{6.5.4}{32}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:53@cref}{{[subsubsection][4][6,5]6.5.4}{[1][32][]32}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:54}{{33}{32}{Input Sufficiency Need Not Preserve Every Declared State}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:54@cref}{{[footnote][33][]33}{[1][32][]32}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:55}{{6.5.4}{32}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:55@cref}{{[subsubsection][4][6,5]6.5.4}{[1][32][]32}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:56}{{34}{32}{Singleton Sufficiency Gives One Conditional Winner}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:56@cref}{{[footnote][34][]34}{[1][32][]32}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:57}{{6.5.4}{32}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:57@cref}{{[subsubsection][4][6,5]6.5.4}{[1][32][]32}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:58}{{35}{32}{Relevance and Positive Support}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:58@cref}{{[footnote][35][]35}{[1][32][]32}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:59}{{6.5.4}{33}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:59@cref}{{[subsubsection][4][6,5]6.5.4}{[1][33][]33}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:5@cref}{{[footnote][3][]3}{[1][6][]6}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:6}{{2.3}{7}{Sufficiency and Relevance}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:60}{{36}{33}{When No Interface Preserves Every Declared State}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:60@cref}{{[footnote][36][]36}{[1][33][]33}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:61}{{6.5.4}{33}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:61@cref}{{[subsubsection][4][6,5]6.5.4}{[1][33][]33}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:62}{{37}{33}{Every Declared Observation Needs a Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:62@cref}{{[footnote][37][]37}{[1][33][]33}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:63}{{6.5.4}{35}{Observation Coverage Adds a Support Witness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:63@cref}{{[subsubsection][4][6,5]6.5.4}{[1][35][]35}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:64}{{38}{35}{Complexity of Preserving Every Declared State}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:64@cref}{{[footnote][38][]38}{[1][35][]35}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:65}{{39}{36}{One Fiber: Equality Versus a Threshold}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:65@cref}{{[footnote][39][]39}{[1][36][]36}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:66}{{6.5.5}{36}{One Fiber: Equality Versus a Threshold}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:66@cref}{{[subsubsection][5][6,5]6.5.5}{[1][36][]36}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:67}{{40}{36}{Finding One Observation with a Unique Winner}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:67@cref}{{[footnote][40][]40}{[1][36][]36}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:68}{{6.5.6}{36}{A Common Counting Source for Two Constructions}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:68@cref}{{[subsubsection][6][6,5]6.5.6}{[1][36][]36}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:69}{{41}{36}{One Threshold for Every Observation}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:69@cref}{{[footnote][41][]41}{[1][36][]36}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:6@cref}{{[subsection][3][2]2.3}{[1][7][]7}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:7}{{4}{7}{On Products, the Necessary Inputs Suffice}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:70}{{6.5.7}{37}{Exact Two-Action Classification}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:70@cref}{{[subsubsection][7][6,5]6.5.7}{[1][37][]37}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:71}{{42}{37}{A Threshold Is a Family of Nonzero Tests}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:71@cref}{{[footnote][42][]42}{[1][37][]37}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:72}{{6.5.7}{37}{Exact Two-Action Classification}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:72@cref}{{[subsubsection][7][6,5]6.5.7}{[1][37][]37}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:73}{{43}{37}{Exact Two-Action Decisiveness Classification}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:73@cref}{{[footnote][43][]43}{[1][37][]37}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:74}{{44}{39}{Which distribution restrictions already preserve hardness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:74@cref}{{[footnote][44][]44}{[1][38][]39}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:75}{{6.6.1}{40}{Succinct Boolean Products: A One-to-$p$ Gap}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:75@cref}{{[subsubsection][1][6,6]6.6.1}{[1][40][]40}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:76}{{45}{40}{Boolean Product One-to-$p$ Gap}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:76@cref}{{[footnote][45][]45}{[1][40][]40}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:77}{{6.6.1}{40}{Succinct Boolean Products: A One-to-$p$ Gap}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:77@cref}{{[subsubsection][1][6,6]6.6.1}{[1][40][]40}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:78}{{46}{40}{One Input or All Inputs: A Hard Approximation Gap}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:78@cref}{{[footnote][46][]46}{[1][40][]40}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:79}{{6.6.1}{41}{Succinct Boolean Products: A One-to-$p$ Gap}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:79@cref}{{[subsubsection][1][6,6]6.6.1}{[1][41][]41}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:7@cref}{{[footnote][4][]4}{[1][7][]7}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:8}{{2.3}{7}{Sufficiency and Relevance}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:80}{{47}{41}{Input-Length Inapproximability}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:80@cref}{{[footnote][47][]47}{[1][41][]41}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:81}{{6.6.2}{41}{Within-Budget Decisiveness Has the Same Worst-Case Gap}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:81@cref}{{[subsubsection][2][6,6]6.6.2}{[1][41][]41}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:82}{{48}{41}{A One-to-All Gap for Within-Budget Decisiveness}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:82@cref}{{[footnote][48][]48}{[1][41][]41}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:83}{{6.6.3}{42}{Explicit Listed Tables: A Logarithmic Guarantee}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:83@cref}{{[subsubsection][3][6,6]6.6.3}{[1][42][]42}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:84}{{49}{42}{Discernibility Hitting-Set Formulation}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:84@cref}{{[footnote][49][]49}{[1][42][]42}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:85}{{6.6.3}{42}{Explicit Listed Tables: A Logarithmic Guarantee}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:85@cref}{{[subsubsection][3][6,6]6.6.3}{[1][42][]42}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:86}{{50}{42}{Cardinality-Preserving Equivalence with Set Cover on the Gadget Family}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:86@cref}{{[footnote][50][]50}{[1][42][]42}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:87}{{51}{42}{Explicit Listed Tables: A Logarithmic Guarantee}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:87@cref}{{[footnote][51][]51}{[1][42][]42}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:88}{{6.7}{43}{Sequential Certification}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:88@cref}{{[subsection][7][6]6.7}{[1][43][]43}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:89}{{52}{43}{Irrelevant Now, Necessary Later}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:89@cref}{{[footnote][52][]52}{[1][43][]43}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:8@cref}{{[subsection][3][2]2.3}{[1][7][]7}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:9}{{5}{7}{Full Interface and Smallest Sufficient Interface}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:90}{{6.7.1}{44}{Sequential Decision Problems}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:90@cref}{{[subsubsection][1][6,7]6.7.1}{[1][44][]44}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:91}{{53}{44}{The Least Sequentially Sufficient Set Is the Relevant Set}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:91@cref}{{[footnote][53][]53}{[1][44][]44}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:92}{{6.7.2}{45}{Bounded Control Alternation}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:92@cref}{{[subsubsection][2][6,7]6.7.2}{[1][45][]45}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:93}{{54}{45}{Bounded-Alternation Certification Ladder}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:93@cref}{{[footnote][54][]54}{[1][45][]45}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:94}{{6.7.2}{45}{Why this holds}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:94@cref}{{[subsubsection][2][6,7]6.7.2}{[1][45][]45}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:95}{{55}{45}{Unbounded-Alternation Limit}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:95@cref}{{[footnote][55][]55}{[1][45][]45}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:96}{{7}{48}{Input Removal in Multistep POMDPs}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:96@cref}{{[section][7][]7}{[1][48][]48}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:97}{{56}{48}{Polynomial-Space Exact Continuation}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:97@cref}{{[footnote][56][]56}{[1][48][]48}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:98}{{7}{48}{Why this holds}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:98@cref}{{[section][7][]7}{[1][48][]48}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:99}{{57}{48}{Sign-Separated QBF Planning Core}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:99@cref}{{[footnote][57][]57}{[1][48][]48}{}{}{}}
\newlabel{paper-claim-location:decision_quotient_jair:9@cref}{{[footnote][5][]5}{[1][7][]7}{}{}{}}
\newlabel{prob:anchor-deployability}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:anchor-deployability@cref}{{[theorem][21][6]6.21}{[1][30][]30}{}{}{}}
\newlabel{prob:anchor-support-relative}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:anchor-support-relative@cref}{{[theorem][21][6]6.21}{[1][29][]30}{}{}{}}
\newlabel{prob:deployability-check}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:deployability-check@cref}{{[theorem][21][6]6.21}{[1][30][]30}{}{}{}}
\newlabel{prob:joint-preservation-check}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:joint-preservation-check@cref}{{[theorem][21][6]6.21}{[1][30][]30}{}{}{}}
\newlabel{prob:minimum-deployable}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:minimum-deployable@cref}{{[theorem][21][6]6.21}{[1][30][]30}{}{}{}}
\newlabel{prob:minimum-support-relative}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:minimum-support-relative@cref}{{[theorem][21][6]6.21}{[1][29][]30}{}{}{}}
\newlabel{prob:stochastic-anchor-preservation}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:stochastic-anchor-preservation@cref}{{[theorem][21][6]6.21}{[1][30][]30}{}{}{}}
\newlabel{prob:stochastic-anchor-sufficiency}{{6.31}{35}{One-Conditional-Winner Queries}{}{}}
\newlabel{prob:stochastic-anchor-sufficiency@cref}{{[theorem][31][6]6.31}{[1][35][]35}{}{}{}}
\newlabel{prob:stochastic-minimum-preservation}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:stochastic-minimum-preservation@cref}{{[theorem][21][6]6.21}{[1][30][]30}{}{}{}}
\newlabel{prob:stochastic-minimum-sufficient}{{6.31}{35}{One-Conditional-Winner Queries}{}{}}
\newlabel{prob:stochastic-minimum-sufficient@cref}{{[theorem][31][6]6.31}{[1][35][]35}{}{}{}}
\newlabel{prob:stochastic-singleton-sufficiency}{{6.31}{35}{One-Conditional-Winner Queries}{}{}}
\newlabel{prob:stochastic-singleton-sufficiency@cref}{{[theorem][31][6]6.31}{[1][35][]35}{}{}{}}
\newlabel{prob:stochastic-sufficiency}{{6.21}{29}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:stochastic-sufficiency@cref}{{[theorem][21][6]6.21}{[1][29][]29}{}{}{}}
\newlabel{prob:support-relative-check}{{6.21}{30}{Preservation and Observation-Coverage Queries}{}{}}
\newlabel{prob:support-relative-check@cref}{{[theorem][21][6]6.21}{[1][29][]30}{}{}{}}
\newlabel{prop:exact-output-realizes-optimizer-quotient}{{2.14}{8}{Admissible Outputs as an Optimizer Quotient}{}{}}
\newlabel{prop:exact-output-realizes-optimizer-quotient@cref}{{[theorem][14][2]2.14}{[1][8][]8}{}{}{}}
\newlabel{prop:joint-preservation-empty}{{6.28}{33}{When No Interface Preserves Every Declared State}{}{}}
\newlabel{prop:joint-preservation-empty@cref}{{[theorem][28][6]6.28}{[1][33][]33}{}{}{}}
\newlabel{prop:listed-discernibility-hitting-set}{{6.42}{42}{Discernibility Hitting-Set Formulation}{}{}}
\newlabel{prop:listed-discernibility-hitting-set@cref}{{[theorem][42][6]6.42}{[1][42][]42}{}{}{}}
\newlabel{prop:minimal-relevant-equiv}{{2.11}{7}{On Products, the Necessary Inputs Suffice}{}{}}
\newlabel{prop:minimal-relevant-equiv@cref}{{[theorem][11][2]2.11}{[1][7][]7}{}{}{}}
\newlabel{prop:paired-family-approximation-gap}{{6.38}{40}{Boolean Product One-to-$p$ Gap}{}{}}
\newlabel{prop:paired-family-approximation-gap@cref}{{[theorem][38][6]6.38}{[1][40][]40}{}{}{}}
\newlabel{prop:pomdp-horizon-two-inheritance}{{7.8}{49}{Horizon-Two Inheritance}{}{}}
\newlabel{prop:pomdp-horizon-two-inheritance@cref}{{[theorem][8][7]7.8}{[1][49][]49}{}{}{}}
\newlabel{prop:preservation-decisiveness-intersection}{{6.18}{28}{Intersection Closure Separates Preservation from Decisiveness}{}{}}
\newlabel{prop:preservation-decisiveness-intersection@cref}{{[theorem][18][6]6.18}{[1][28][]28}{}{}{}}
\newlabel{prop:sequential-minimal-relevant}{{6.48}{44}{The Least Sequentially Sufficient Set Is the Relevant Set}{}{}}
\newlabel{prop:sequential-minimal-relevant@cref}{{[theorem][48][6]6.48}{[1][44][]44}{}{}{}}
\newlabel{prop:static-not-stochastic}{{6.25}{32}{Input Sufficiency Need Not Preserve Every Declared State}{}{}}
\newlabel{prop:static-not-stochastic@cref}{{[theorem][25][6]6.25}{[1][32][]32}{}{}{}}
\newlabel{prop:static-to-stochastic-product}{{6.26}{32}{Singleton Sufficiency Gives One Conditional Winner}{}{}}
\newlabel{prop:static-to-stochastic-product@cref}{{[theorem][26][6]6.26}{[1][32][]32}{}{}{}}
\newlabel{prop:stochastic-not-sequential}{{6.45}{43}{Irrelevant Now, Necessary Later}{}{}}
\newlabel{prop:stochastic-not-sequential@cref}{{[theorem][45][6]6.45}{[1][43][]43}{}{}{}}
\newlabel{prop:two-action-exact-counting}{{6.35}{37}{Exact Two-Action Decisiveness Classification}{}{}}
\newlabel{prop:two-action-exact-counting@cref}{{[theorem][35][6]6.35}{[1][37][]37}{}{}{}}
\newlabel{rem:listed-product-closure}{{2.13}{7}{Listed States and Product Closure}{}{}}
\newlabel{rem:listed-product-closure@cref}{{[theorem][13][2]2.13}{[1][7][]7}{}{}{}}
\newlabel{rem:nested-class-not-simplified}{{6.36}{38}{Why the nested class is not simplified}{}{}}
\newlabel{rem:nested-class-not-simplified@cref}{{[theorem][36][6]6.36}{[1][38][]38}{}{}{}}
\newlabel{rem:product-closure-scope}{{3.2}{11}{Product-Closure Scope}{}{}}
\newlabel{rem:product-closure-scope@cref}{{[theorem][2][3]3.2}{[1][11][]11}{}{}{}}
\newlabel{rem:rough-set-search-collapse}{{6.8}{23}{Rough-Set Search versus Product-Closed Certification}{}{}}
\newlabel{rem:rough-set-search-collapse@cref}{{[theorem][8][6]6.8}{[1][23][]23}{}{}{}}
\newlabel{sec:approximation-across-presentations}{{6.6}{39}{Approximation Across Presentations}{}{}}
\newlabel{sec:approximation-across-presentations@cref}{{[subsection][6][6]6.6}{[1][39][]39}{}{}{}}
\newlabel{sec:certification-complexity}{{6}{19}{Certification Complexity}{}{}}
\newlabel{sec:certification-complexity@cref}{{[section][6][]6}{[1][19][]19}{}{}{}}
\newlabel{sec:complexity-labels}{{5.1}{18}{Choosing Inputs and Checking States}{}{}}
\newlabel{sec:complexity-labels@cref}{{[subsection][1][5]5.1}{[1][18][]18}{}{}{}}
\newlabel{sec:contribution-boundary}{{5.2}{18}{Relation to Existing Complexity Results}{}{}}
\newlabel{sec:contribution-boundary@cref}{{[subsection][2][5]5.2}{[1][18][]18}{}{}{}}
\newlabel{sec:data-code-availability}{{11}{54}{Data and Code Availability}{}{}}
\newlabel{sec:data-code-availability@cref}{{[section][11][]11}{[1][54][]54}{}{}{}}
\newlabel{sec:dichotomy}{{3}{9}{Encodings and Access Models}{}{}}
\newlabel{sec:dichotomy@cref}{{[section][3][]3}{[1][9][]9}{}{}{}}
\newlabel{sec:encoding}{{3}{9}{Encodings and Access Models}{}{}}
\newlabel{sec:encoding@cref}{{[section][3][]3}{[1][9][]9}{}{}{}}
\newlabel{sec:formal-setup}{{2}{4}{What Input Removal Must Preserve}{}{}}
\newlabel{sec:formal-setup@cref}{{[section][2][]2}{[1][4][]4}{}{}{}}
\newlabel{sec:hardness}{{6.1}{20}{Input Sufficiency: Product Closure Versus Missing Combinations}{}{}}
\newlabel{sec:hardness@cref}{{[subsection][1][6]6.1}{[1][20][]20}{}{}{}}
\newlabel{sec:introduction}{{1}{1}{Introduction}{}{}}
\newlabel{sec:introduction@cref}{{[section][1][]1}{[1][1][]1}{}{}{}}
\newlabel{sec:learned-policy-audit}{{4.4.2}{17}{Auditing the Same Classifier on Two State Domains}{}{}}
\newlabel{sec:learned-policy-audit@cref}{{[subsubsection][2][4,4]4.4.2}{[1][16][]17}{}{}{}}
\newlabel{sec:multistep-pomdp}{{7}{45}{Input Removal in Multistep POMDPs}{}{}}
\newlabel{sec:multistep-pomdp@cref}{{[section][7][]7}{[1][45][]45}{}{}{}}
\newlabel{sec:open-problems}{{10}{52}{Open Problems}{}{}}
\newlabel{sec:open-problems@cref}{{[section][10][]10}{[1][52][]52}{}{}{}}
\newlabel{sec:preflight}{{4.4.1}{16}{Contract and Checks}{}{}}
\newlabel{sec:preflight@cref}{{[subsubsection][1][4,4]4.4.1}{[1][16][]16}{}{}{}}
\newlabel{sec:regime-hierarchy}{{6.4}{28}{Intersection Closure Governs Within-Budget Certification}{}{}}
\newlabel{sec:regime-hierarchy@cref}{{[subsection][4][6]6.4}{[1][28][]28}{}{}{}}
\newlabel{sec:results-overview}{{5}{18}{What Must Be Proved Before Removing an Input}{}{}}
\newlabel{sec:results-overview@cref}{{[section][5][]5}{[1][18][]18}{}{}{}}
\newlabel{sec:sequential}{{6.7}{43}{Sequential Certification}{}{}}
\newlabel{sec:sequential@cref}{{[subsection][7][6]6.7}{[1][42][]43}{}{}{}}
\newlabel{sec:stochastic}{{6.5}{29}{Stochastic Certification}{}{}}
\newlabel{sec:stochastic-contracts}{{6.2}{24}{What to Require at Unreachable Observations}{}{}}
\newlabel{sec:stochastic-contracts@cref}{{[subsection][2][6]6.2}{[1][24][]24}{}{}{}}
\newlabel{sec:stochastic@cref}{{[subsection][5][6]6.5}{[1][29][]29}{}{}{}}
\newlabel{sec:structural-consequences}{{4.4}{16}{An Audit Procedure}{}{}}
\newlabel{sec:structural-consequences@cref}{{[subsection][4][4]4.4}{[1][15][]16}{}{}{}}
\newlabel{sec:tract-separable}{{4.1}{11}{Two Direct Decomposition Checks}{}{}}
\newlabel{sec:tract-separable@cref}{{[subsection][1][4]4.1}{[1][11][]11}{}{}{}}
\newlabel{sec:tract-symmetry}{{4.3}{14}{Coordinate Symmetry and Histogram Certificates}{}{}}
\newlabel{sec:tract-symmetry@cref}{{[subsection][3][4]4.3}{[1][13][]14}{}{}{}}
\newlabel{sec:tract-tensor}{{4.1}{11}{Two Direct Decomposition Checks}{}{}}
\newlabel{sec:tract-tensor@cref}{{[subsection][1][4]4.1}{[1][11][]11}{}{}{}}
\newlabel{sec:tract-treewidth}{{4.2}{12}{Bounded Treewidth}{}{}}
\newlabel{sec:tract-treewidth@cref}{{[subsection][2][4]4.2}{[1][12][]12}{}{}{}}
\newlabel{sec:tractable}{{4}{11}{Algorithms and Structural Certificates}{}{}}
\newlabel{sec:tractable@cref}{{[section][4][]4}{[1][11][]11}{}{}{}}
\newlabel{sec:two-action-exact}{{6.5.7}{37}{Exact Two-Action Classification}{}{}}
\newlabel{sec:two-action-exact@cref}{{[subsubsection][7][6,5]6.5.7}{[1][37][]37}{}{}{}}
\newlabel{sec:verification-scope}{{9}{51}{Verification Scope}{}{}}
\newlabel{sec:verification-scope@cref}{{[section][9][]9}{[1][51][]51}{}{}{}}
\newlabel{tab:central-questions}{{2}{19}{Four input-removal questions. The first is the baseline; the other three expose coordinate choice, support coverage, and weighted comparison. These are decision problems under the stated succinct models, not runtime predictions for individual instances. The full classifications appear in Table~\ref {tab:regime-matrix}}{}{}}
\newlabel{tab:central-questions@cref}{{[table][2][]2}{[1][18][]19}{}{}{}}
\newlabel{tab:multistep-contracts}{{4}{46}{Multistep scopes and contracts. Scope specifies when to test; the contract specifies which histories and support obligations to include}{}{}}
\newlabel{tab:multistep-contracts@cref}{{[table][4][]4}{[1][46][]46}{}{}{}}
\newlabel{tab:regime-matrix}{{5}{51}{Static and one-step stochastic classifications for the displayed succinct encodings. Product closure supplies one least sufficient interface; missing support can restore incomparable blanket choices; observation coverage adds a support witness; decisiveness retains weighted score comparison. For a fixed retained input set, a some-observation query asks whether at least one realized observation satisfies the row predicate. Semantic validity promises use Definition~\ref {def:validity-promise-convention}}{}{}}
\newlabel{tab:regime-matrix@cref}{{[table][5][]5}{[1][50][]51}{}{}{}}
\newlabel{tab:sequential-matrix}{{6}{51}{Sequential extension. A fixed bound on controller--environment move blocks determines the polynomial-hierarchy level. When that bound grows with the input, or a unary-horizon POMDP updates beliefs after observations, the corresponding certification problems are PSPACE-complete. Here $d$ is fixed, the block bound is promised, and $\Sigma _0^P=\Pi _0^P=\mathsf P$. The multistep row covers root-only and historywise preservation, observation coverage, and decisiveness; no some-observation query is posed}{}{}}
\newlabel{tab:sequential-matrix@cref}{{[table][6][]6}{[1][50][]51}{}{}{}}
\newlabel{tab:support-contract-guide}{{3}{26}{What each requirement asks. Under full support the four preservation rows coincide; one conditional winner still asks a different question. On a zero-mass fiber the score rule gives every action score zero}{}{}}
\newlabel{tab:support-contract-guide@cref}{{[table][3][]3}{[1][25][]26}{}{}{}}
\newlabel{tab:tractability-map}{{1}{12}{Algorithms and certified structural reductions. The first row is an explicit-input baseline; the remaining rows state sufficient structure or certificate data}{}{}}
\newlabel{tab:tractability-map@cref}{{[table][1][]1}{[1][11][]12}{}{}{}}
\newlabel{thm:anchor-sigma2p}{{6.9}{23}{Finding One Observation That Preserves the Answer}{}{}}
\newlabel{thm:anchor-sigma2p@cref}{{[theorem][9][6]6.9}{[1][23][]23}{}{}{}}
\newlabel{thm:listed-minsuff-sigma2p}{{6.7}{21}{Missing Combinations Keep the Choice Alive}{}{}}
\newlabel{thm:listed-minsuff-sigma2p@cref}{{[theorem][7][6]6.7}{[1][21][]21}{}{}{}}
\newlabel{thm:master-factorization}{{2.6}{5}{Kernel Factorization for the Optimizer Map}{}{}}
\newlabel{thm:master-factorization@cref}{{[theorem][6][2]2.6}{[1][5][]5}{}{}{}}
\newlabel{thm:minimum-decisiveness-approximation-threshold}{{6.41}{41}{A One-to-All Gap for Within-Budget Decisiveness}{}{}}
\newlabel{thm:minimum-decisiveness-approximation-threshold@cref}{{[theorem][41][6]6.41}{[1][41][]41}{}{}{}}
\newlabel{thm:minsuff-conp}{{6.6}{21}{Finding a Sufficient Set Within Budget Is coNP-Complete}{}{}}
\newlabel{thm:minsuff-conp@cref}{{[theorem][6][6]6.6}{[1][21][]21}{}{}{}}
\newlabel{thm:optimizer-markov-blanket}{{6.15}{27}{Optimizer Markov-Blanket Equivalence}{}{}}
\newlabel{thm:optimizer-markov-blanket@cref}{{[theorem][15][6]6.15}{[1][27][]27}{}{}{}}
\newlabel{thm:pomdp-exact-pspace}{{7.7}{49}{Unary-Horizon Interface Certification Is PSPACE-Complete}{}{}}
\newlabel{thm:pomdp-exact-pspace@cref}{{[theorem][7][7]7.7}{[1][49][]49}{}{}{}}
\newlabel{thm:sequential-anchor-hard}{{6.50}{45}{Unbounded-Alternation Limit}{}{}}
\newlabel{thm:sequential-anchor-hard@cref}{{[theorem][50][6]6.50}{[1][45][]45}{}{}{}}
\newlabel{thm:sequential-bounded-ladder}{{6.49}{45}{Bounded-Alternation Certification Ladder}{}{}}
\newlabel{thm:sequential-bounded-ladder@cref}{{[theorem][49][6]6.49}{[1][45][]45}{}{}{}}
\newlabel{thm:sequential-minimum-hard}{{6.50}{45}{Unbounded-Alternation Limit}{}{}}
\newlabel{thm:sequential-minimum-hard@cref}{{[theorem][50][6]6.50}{[1][45][]45}{}{}{}}
\newlabel{thm:sequential-pspace}{{6.50}{45}{Unbounded-Alternation Limit}{}{}}
\newlabel{thm:sequential-pspace@cref}{{[theorem][50][6]6.50}{[1][45][]45}{}{}{}}
\newlabel{thm:set-cover-cardinality-equivalence}{{6.43}{42}{Cardinality-Preserving Equivalence with Set Cover on the Gadget Family}{}{}}
\newlabel{thm:set-cover-cardinality-equivalence@cref}{{[theorem][43][6]6.43}{[1][42][]42}{}{}{}}
\newlabel{thm:stochastic-anchor-hard}{{6.32}{36}{Finding One Observation with a Unique Winner}{}{}}
\newlabel{thm:stochastic-anchor-hard@cref}{{[theorem][32][6]6.32}{[1][36][]36}{}{}{}}
\newlabel{thm:stochastic-preservation-full-support-variants}{{6.23}{31}{Full Support Reduces Preservation to Input Sufficiency}{}{}}
\newlabel{thm:stochastic-preservation-full-support-variants@cref}{{[theorem][23][6]6.23}{[1][31][]31}{}{}{}}
\newlabel{thm:stochastic-preservation-tight}{{6.29}{33}{Every Declared Observation Needs a Witness}{}{}}
\newlabel{thm:stochastic-preservation-tight@cref}{{[theorem][29][6]6.29}{[1][33][]33}{}{}{}}
\newlabel{thm:stochastic-preservation-zero-mass-characterization}{{6.24}{31}{Preservation Can Hold Without Observation Coverage}{}{}}
\newlabel{thm:stochastic-preservation-zero-mass-characterization@cref}{{[theorem][24][6]6.24}{[1][31][]31}{}{}{}}
\newlabel{thm:succinct-product-approximation-threshold}{{6.39}{40}{One Input or All Inputs: A Hard Approximation Gap}{}{}}
\newlabel{thm:succinct-product-approximation-threshold@cref}{{[theorem][39][6]6.39}{[1][40][]40}{}{}{}}
\newlabel{thm:sufficiency-conp}{{6.5}{20}{One-Coordinate Deletion Is coNP-Complete}{}{}}
\newlabel{thm:sufficiency-conp@cref}{{[theorem][5][6]6.5}{[1][20][]20}{}{}{}}
\newlabel{thm:support-relative-blanket-classification}{{6.22}{30}{Sparse Support Keeps the Blanket Choice Alive}{}{}}
\newlabel{thm:support-relative-blanket-classification@cref}{{[theorem][22][6]6.22}{[1][30][]30}{}{}{}}
\newlabel{thm:symmetric-complexity}{{4.3}{15}{Orbit Representatives and the Histogram Certificate}{}{}}
\newlabel{thm:symmetric-complexity@cref}{{[theorem][3][4]4.3}{[1][15][]15}{}{}{}}
\newlabel{thm:treewidth}{{4.1}{12}{Bounded-Width CSP for Violating State Pairs}{}{}}
\newlabel{thm:treewidth@cref}{{[theorem][1][4]4.1}{[1][12][]12}{}{}{}}
\makeatother


==> lean-handle-macros.tex <==
% Auto-generated by scripts/build_papers.py. Do not edit manually.
% Lean handle macro definitions: compact footnote markers in body text
\providecommand{\LH}[1]{}
\renewcommand{\LH}[1]{\leavevmode\nobreak\mbox{\ttfamily\nolinkurl{#1}}}
\providecommand{\LHrng}[3]{}
\renewcommand{\LHrng}[3]{\leavevmode\nobreak\mbox{\ttfamily\nolinkurl{#1#2-#3}}}
\newif\ifleanmetaseen
\leanmetaseenfalse
\providecommand{\leanfootnoteterminator}{}
\providecommand{\leanfootnoteformat}[1]{#1}
\makeatletter
\providecommand{\PaperClaimLocationRecord}[2]{}
\newcounter{PaperClaimLocationIndex}
\newcommand{\PaperRecordClaimLocation}[1]{\stepcounter{PaperClaimLocationIndex}\label{paper-claim-location:\jobname:\thePaperClaimLocationIndex}\protected@write\@auxout{}{\string\PaperClaimLocationRecord{\thePaperClaimLocationIndex}{\detokenize{#1}}}}
\NewDocumentCommand{\PaperIndexedFootnote}{o +m}{\IfNoValueTF{#1}{\PaperOriginalFootnote{\PaperRecordClaimLocation{#2}#2}}{\PaperOriginalFootnote[#1]{\PaperRecordClaimLocation{#2}#2}}}
\AddToHook{begindocument/end}{\let\PaperOriginalFootnote\footnote\let\footnote\PaperIndexedFootnote}
\providecommand{\leanmetapendinghandles}{}
\global\let\leanmetapendinghandles\@empty
\providecommand{\leanmetapending}[1]{}
\renewcommand{\leanmetapending}[1]{\def\leanmetatest{#1}\ifx\leanmetatest\@empty\global\let\leanmetapendinghandles\@empty\else\PaperRecordClaimLocation{#1}\gdef\leanmetapendinghandles{#1}\fi}
\providecommand{\leanmetaproofpendinghandles}{}
\global\let\leanmetaproofpendinghandles\@empty
\providecommand{\leanmetaproofpending}[1]{}
\renewcommand{\leanmetaproofpending}[1]{\def\leanmetatest{#1}\ifx\leanmetatest\@empty\global\let\leanmetaproofpendinghandles\@empty\else\gdef\leanmetaproofpendinghandles{#1}\fi}
\providecommand{\leanmetaheadmark}{}
\newif\ifleanmetaheadprinted
\leanmetaheadprintedfalse
\renewcommand{\leanmetaheadmark}{\ifx\leanmetapendinghandles\@empty\else\nobreak\hspace{0.2em}\footnote{\leanfootnoteformat{\strut\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi\leanmetapendinghandles}}\global\leanmetaheadprintedtrue\fi}
\providecommand{\leanmetaheadtext}{}
\renewcommand{\leanmetaheadtext}{\ifleanmetaheadprinted\global\let\leanmetapendinghandles\@empty\global\leanmetaheadprintedfalse\fi}
\providecommand{\leanmetaproofmark}{}
\renewcommand{\leanmetaproofmark}{\ifx\leanmetaproofpendinghandles\@empty\else\ifhmode\unskip\fi\footnote{\leanfootnoteformat{\strut\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi\leanmetaproofpendinghandles\leanfootnoteterminator}}\global\let\leanmetaproofpendinghandles\@empty\fi}
\@ifundefined{newtheoremstyle}{}{\@ifundefined{thmname}{}{%
  \newtheoremstyle{leanplain}
    {6pt}{6pt}{\itshape}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}\leanmetaheadmark\leanmetaheadtext}
  \newtheoremstyle{leandefinition}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}\leanmetaheadmark\leanmetaheadtext}
  \newtheoremstyle{leandef}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}\leanmetaheadmark\leanmetaheadtext}
  \newtheoremstyle{leanremark}
    {6pt}{6pt}{}{}{\bfseries}{.}{ }
    {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}\leanmetaheadmark\leanmetaheadtext}
}}
\@ifundefined{thm@thmcaption}{}{\@ifundefined{@opargbegintheorem}{}{%
  \def\@xthm#1#2#3{%
    \@begintheorem{#3}{\csname the#2\endcsname\leanmetaheadmark}%
    \leanmetaheadtext
    \ifx\thm@starredenv\@undefined
      \thm@thmcaption{#1}{{#3}{\csname the#2\endcsname}{}}\fi
    \ignorespaces}
  \def\@ythm#1#2#3[#4]{%
    \expandafter\global\expandafter\def\csname#1name\endcsname{#4}%
    \@opargbegintheorem{#3}{\csname the#2\endcsname}{#4\leanmetaheadmark}%
    \leanmetaheadtext
    \ifx\thm@starredenv\@undefined
      \thm@thmcaption{#1}{{#3}{\csname the#2\endcsname}{#4}}\fi
    \ignorespaces}
}}
\makeatother
\providecommand{\leanmeta}[1]{}
\renewcommand{\leanmeta}[1]{\ifhmode\unskip\fi\footnote{\leanfootnoteformat{\strut\ifleanmetaseen\else Lean: \global\leanmetaseentrue\fi#1\leanfootnoteterminator}}}

